A genus-zero surface with bounded curvature enclosing less volume than the unit sphere

We produce a family of bodies in $\mathbb R^3$ parameterized by $\varepsilon > 0$, each bounded by a smooth topological sphere with principal curvatures in $[-1, 1]$, and having volume arbitrarily close to $ 16 - 4\sqrt 3 + \left(10 \sqrt 3 - 14\right) \pi - \left(\frac{10}{3} - \sqrt 3\right) \pi^2 \approx 3.70.$ Thus, in contrast to the two-dimensional case, the unit sphere (which bounds a ball of volume $\frac{4 }{ 3} \pi \approx 4.19$) does not enclose the minimal volume among all smooth spheres in $\mathbb R^3$ with principal curvatures in $[-1,1]$. This answers a folklore question of Dmitri Burago and Anton Petrunin.

==> adjacency_graph.tex <==
\begin{figure}
\caption{Adjacency graph for the surfaces}
    \label{fig:placeholder}
\begin{center}
\begin{tikzpicture}[scale=1, transform shape]
\tikzstyle{every node}=[circle, draw, inner sep=0.5pt, minimum size=5pt];
\node (n0) at (3.315, 6.376) {0};
\node (n6) at (3.973, 7.512) {6};
\node (n47) at (1.901, 5.943) {47};
\node (n2) at (4.463, 5.894) {2};
\node (n1) at (-2.709, 6.679) {1};
\node (n7) at (-3.266, 7.873) {7};
\node (n45) at (-1.337, 6.109) {45};
\node (n3) at (-3.930, 6.320) {3};
\node (n4) at (4.946, 6.746) {4};
\node (n40) at (3.233, 5.390) {40};
\node (n8) at (5.019, 7.270) {8};
\node (n5) at (-4.328, 7.215) {5};
\node (n41) at (-2.756, 5.698) {41};
\node (n9) at (-4.341, 7.745) {9};
\node (n11) at (3.841, 6.526) {11};
\node (n12) at (-3.247, 6.895) {12};
\node (n10) at (2.716, 7.044) {10};
\node (n13) at (-2.047, 7.276) {13};
\node (n43) at (1.573, 7.599) {43};
\node (n31) at (3.206, 5.975) {31};
\node (n33) at (-2.719, 6.263) {33};
\node (n42) at (-0.868, 7.727) {42};
\node (n14) at (0.342, 7.034) {14};
\node (n25) at (0.375, 8.264) {25};
\node (n46) at (0.281, 5.758) {46};
\node (n15) at (-1.040, 4.508) {15};
\node (n44) at (0.250, 4.453) {44};
\node (n35) at (-0.956, 5.551) {35};
\node (n16) at (-2.139, 5.193) {16};
\node (n23) at (0.017, 3.948) {23};
\node (n36) at (-1.738, 6.548) {36};
\node (n17) at (1.359, 4.387) {17};
\node (n37) at (1.353, 5.446) {37};
\node (n18) at (2.528, 4.968) {18};
\node (n38) at (2.252, 6.356) {38};
\node (n19) at (-0.705, 6.872) {19};
\node (n39) at (0.272, 7.417) {39};
\node (n20) at (-1.366, 8.016) {20};
\node (n24) at (0.212, 6.265) {24};
\node (n27) at (-0.678, 8.781) {27};
\node (n34) at (-1.680, 8.990) {34};
\node (n21) at (1.229, 6.778) {21};
\node (n22) at (2.037, 7.841) {22};
\node (n28) at (1.462, 8.672) {28};
\node (n32) at (2.469, 8.779) {32};
\node (n51) at (-0.357, 2.885) {51};
\node (n26) at (0.142, 5.052) {26};
\node (n29) at (-1.959, 7.738) {29};
\node (n30) at (2.620, 7.507) {30};
\node (n50) at (0.474, 3.157) {50};
\node (n48) at (0.588, 0.896) {48};
\node (n49) at (-0.525, 0.677) {49};
\node (n54) at (0.572, -0.191) {54};
\node (n53) at (0.561, 2.002) {53};
\node (n55) at (-0.510, -0.430) {55};
\node (n52) at (-0.489, 1.779) {52};
\node (n59) at (0.435, -1.265) {59};
\node (n58) at (-0.419, -1.578) {58};
\node (n56) at (-0.131, -2.913) {56};
\node (n57) at (-0.075, -4.292) {57};
\node (n61) at (-1.310, -2.722) {61};
\node (n62) at (1.029, -2.769) {62};
\node (n73) at (1.187, -4.618) {73};
\node (n67) at (-1.389, -4.510) {67};
\node (n66) at (-0.114, -5.725) {66};
\node (n60) at (-0.082, -2.251) {60};
\node (n63) at (-0.418, -3.190) {63};
\node (n77) at (-2.202, -3.699) {77};
\node (n81) at (-1.984, -3.074) {81};
\node (n76) at (1.874, -3.792) {76};
\node (n89) at (1.239, -3.337) {89};
\node (n90) at (-0.605, -4.253) {90};
\node (n64) at (1.694, -7.985) {64};
\node (n72) at (0.999, -6.914) {72};
\node (n101) at (2.539, -8.883) {101};
\node (n97) at (0.678, -9.159) {97};
\node (n93) at (1.210, -7.777) {93};
\node (n65) at (-2.350, -7.827) {65};
\node (n105) at (-3.309, -8.627) {105};
\node (n69) at (-1.814, -6.849) {69};
\node (n99) at (-1.667, -8.908) {99};
\node (n91) at (-1.318, -7.977) {91};
\node (n71) at (1.289, -5.866) {71};
\node (n68) at (-1.513, -5.755) {68};
\node (n92) at (-0.028, -7.162) {92};
\node (n79) at (-2.549, -5.003) {79};
\node (n78) at (-2.138, -5.925) {78};
\node (n70) at (-0.497, -7.266) {70};
\node (n98) at (-0.480, -8.490) {98};
\node (n80) at (-0.622, -6.200) {80};
\node (n75) at (1.923, -5.151) {75};
\node (n74) at (0.850, -5.934) {74};
\node (n86) at (0.625, -4.856) {86};
\node (n87) at (1.862, -4.334) {87};
\node (n88) at (2.567, -3.612) {88};
\node (n82) at (-3.120, -3.355) {82};
\node (n83) at (-1.885, -4.820) {83};
\node (n84) at (-2.776, -4.149) {84};
\node (n85) at (-0.650, -5.120) {85};
\node (n104) at (-2.399, -8.748) {104};
\node (n96) at (-1.007, -9.263) {96};
\node (n95) at (0.083, -8.354) {95};
\node (n103) at (2.600, -8.200) {103};
\node (n94) at (1.235, -8.934) {94};
\node (n100) at (2.317, -9.558) {100};
\node (n107) at (-2.076, -10.000) {107};
\node (n102) at (1.628, -9.985) {102};
\node (n106) at (-2.683, -9.660) {106};
\node (n109) at (3.312, -9.590) {109};
\node (n108) at (-3.458, -9.789) {108};
\draw (n0) -- (n6);
\draw (n0) -- (n47);
\draw (n0) -- (n2);
\draw (n6) -- (n4);
\draw (n6) -- (n10);
\draw (n6) -- (n8);
\draw (n47) -- (n10);
\draw (n47) -- (n40);
\draw (n47) -- (n46);
\draw (n2) -- (n4);
\draw (n2) -- (n40);
\draw (n2) -- (n8);
\draw (n1) -- (n7);
\draw (n1) -- (n45);
\draw (n1) -- (n3);
\draw (n7) -- (n5);
\draw (n7) -- (n13);
\draw (n7) -- (n9);
\draw (n45) -- (n13);
\draw (n45) -- (n41);
\draw (n45) -- (n46);
\draw (n3) -- (n5);
\draw (n3) -- (n41);
\draw (n3) -- (n9);
\draw (n4) -- (n11);
\draw (n40) -- (n11);
\draw (n40) -- (n18);
\draw (n5) -- (n12);
\draw (n41) -- (n12);
\draw (n41) -- (n16);
\draw (n11) -- (n10);
\draw (n11) -- (n31);
\draw (n12) -- (n33);
\draw (n12) -- (n13);
\draw (n10) -- (n43);
\draw (n13) -- (n42);
\draw (n43) -- (n14);
\draw (n43) -- (n28);
\draw (n43) -- (n30);
\draw (n31) -- (n18);
\draw (n31) -- (n30);
\draw (n33) -- (n16);
\draw (n33) -- (n29);
\draw (n42) -- (n14);
\draw (n42) -- (n27);
\draw (n42) -- (n29);
\draw (n14) -- (n25);
\draw (n14) -- (n46);
\draw (n25) -- (n28);
\draw (n25) -- (n27);
\draw (n25) -- (n39);
\draw (n46) -- (n44);
\draw (n15) -- (n44);
\draw (n15) -- (n35);
\draw (n15) -- (n16);
\draw (n15) -- (n23);
\draw (n44) -- (n17);
\draw (n44) -- (n50);
\draw (n35) -- (n19);
\draw (n35) -- (n26);
\draw (n35) -- (n36);
\draw (n16) -- (n36);
\draw (n23) -- (n17);
\draw (n23) -- (n51);
\draw (n23) -- (n26);
\draw (n36) -- (n20);
\draw (n36) -- (n29);
\draw (n17) -- (n37);
\draw (n17) -- (n18);
\draw (n37) -- (n21);
\draw (n37) -- (n26);
\draw (n37) -- (n38);
\draw (n18) -- (n38);
\draw (n38) -- (n22);
\draw (n38) -- (n30);
\draw (n19) -- (n39);
\draw (n19) -- (n20);
\draw (n19) -- (n24);
\draw (n39) -- (n21);
\draw (n39) -- (n24);
\draw (n20) -- (n27);
\draw (n20) -- (n34);
\draw (n24) -- (n21);
\draw (n24) -- (n26);
\draw (n27) -- (n34);
\draw (n34) -- (n29);
\draw (n21) -- (n22);
\draw (n22) -- (n28);
\draw (n22) -- (n32);
\draw (n28) -- (n32);
\draw (n32) -- (n30);
\draw (n51) -- (n50);
\draw (n51) -- (n52);
\draw (n50) -- (n53);
\draw (n48) -- (n49);
\draw (n48) -- (n54);
\draw (n48) -- (n53);
\draw (n49) -- (n55);
\draw (n49) -- (n52);
\draw (n54) -- (n55);
\draw (n54) -- (n59);
\draw (n53) -- (n52);
\draw (n55) -- (n58);
\draw (n59) -- (n58);
\draw (n59) -- (n60);
\draw (n58) -- (n56);
\draw (n56) -- (n57);
\draw (n56) -- (n61);
\draw (n56) -- (n62);
\draw (n57) -- (n73);
\draw (n57) -- (n67);
\draw (n57) -- (n66);
\draw (n61) -- (n60);
\draw (n61) -- (n77);
\draw (n61) -- (n81);
\draw (n62) -- (n60);
\draw (n62) -- (n76);
\draw (n62) -- (n89);
\draw (n73) -- (n71);
\draw (n73) -- (n76);
\draw (n67) -- (n77);
\draw (n67) -- (n68);
\draw (n66) -- (n71);
\draw (n66) -- (n68);
\draw (n66) -- (n92);
\draw (n60) -- (n63);
\draw (n63) -- (n89);
\draw (n63) -- (n81);
\draw (n63) -- (n90);
\draw (n77) -- (n79);
\draw (n77) -- (n82);
\draw (n81) -- (n84);
\draw (n81) -- (n82);
\draw (n76) -- (n75);
\draw (n76) -- (n88);
\draw (n89) -- (n87);
\draw (n89) -- (n88);
\draw (n90) -- (n83);
\draw (n90) -- (n85);
\draw (n90) -- (n86);
\draw (n64) -- (n72);
\draw (n64) -- (n101);
\draw (n64) -- (n97);
\draw (n64) -- (n93);
\draw (n72) -- (n70);
\draw (n72) -- (n71);
\draw (n72) -- (n74);
\draw (n101) -- (n102);
\draw (n101) -- (n103);
\draw (n101) -- (n109);
\draw (n97) -- (n94);
\draw (n97) -- (n102);
\draw (n97) -- (n98);
\draw (n93) -- (n92);
\draw (n93) -- (n103);
\draw (n93) -- (n94);
\draw (n65) -- (n105);
\draw (n65) -- (n69);
\draw (n65) -- (n99);
\draw (n65) -- (n91);
\draw (n105) -- (n104);
\draw (n105) -- (n106);
\draw (n105) -- (n108);
\draw (n69) -- (n68);
\draw (n69) -- (n78);
\draw (n69) -- (n70);
\draw (n99) -- (n96);
\draw (n99) -- (n98);
\draw (n99) -- (n106);
\draw (n91) -- (n104);
\draw (n91) -- (n92);
\draw (n91) -- (n96);
\draw (n71) -- (n75);
\draw (n68) -- (n79);
\draw (n92) -- (n95);
\draw (n79) -- (n78);
\draw (n79) -- (n84);
\draw (n78) -- (n80);
\draw (n78) -- (n83);
\draw (n70) -- (n98);
\draw (n70) -- (n80);
\draw (n98) -- (n95);
\draw (n80) -- (n74);
\draw (n80) -- (n85);
\draw (n75) -- (n74);
\draw (n75) -- (n87);
\draw (n74) -- (n86);
\draw (n86) -- (n85);
\draw (n86) -- (n87);
\draw (n87) -- (n88);
\draw (n82) -- (n84);
\draw (n83) -- (n84);
\draw (n83) -- (n85);
\draw (n104) -- (n107);
\draw (n96) -- (n95);
\draw (n96) -- (n107);
\draw (n95) -- (n94);
\draw (n103) -- (n100);
\draw (n94) -- (n100);
\draw (n100) -- (n102);
\draw (n100) -- (n109);
\draw (n107) -- (n106);
\draw (n107) -- (n108);
\end{tikzpicture}

\end{center}
\end{figure}
